One Shot Learning for Edge Detection on Point Clouds

Each scanner possesses its unique characteristics and exhibits its distinct sampling error distribution. Training a network on a dataset that includes data collected from different scanners is less effective than training it on data specific to a single scanner. Therefore, we present a novel one-shot learning method allowing for edge extraction on point clouds, by learning the specific data distribution of the target point cloud, and thus achieve superior results compared to networks that were trained on general data distributions. More specifically, we present how to train a lightweight network named OSFENet (One-Shot edge Feature Extraction Network), by designing a filtered-KNN-based surface patch representation that supports a one-shot learning framework. Additionally, we introduce an RBF_DoS module, which integrates Radial Basis Function-based Descriptor of the Surface patch, highly beneficial for the edge extraction on point clouds. The advantage of the proposed OSFENet is demonstrated through comparative analyses against 7 baselines on the ABC dataset, and its practical utility is validated by results across diverse real-scanned datasets, including indoor scenes like S3DIS dataset, and outdoor scenes such as the Semantic3D dataset and UrbanBIS dataset.

==> 10._application.tex <==
\section{Application}


\begin{figure*}
  \centering
  \includegraphics[width=\linewidth]{Figure/limitation_shrec.pdf}
  \caption{The results of OSFENet, EC-Net\cite{Yu2018ECNet}, and NerVE\cite{Nerve2023CVPR} on the SHREC dataset\cite{Thompson2019FeatureCE}.}
  \label{fig:limitation}
\end{figure*}


Excluding surface segmentation, a wide range of applications that rely on features can benefit from this approach. We summarize the other applications in the following three areas: (i) Point cloud simplification: should retain both sharp and smooth features, large-scale and detailed elements, as well as structural and textural characteristics, while removing non-features. Therefore, our method can be employed as an up-stream technique for point cloud simplification; (ii) Model editing: refers to the process of modifying or altering a 3D model's geometry or appearance, for example, adjusting textures or materials, or refining details for a specific purpose. Therefore, our method can segment the model into finer grains, assisting the user in efficiently selecting elements, such as specific faces on a building. (3) Line drawing generation: is an important method of non-photorealistic rendering in computer graphics, as line drawings (also referred to as sketches) can better communicate main visual information. For example, from Figure\ref{fig:indoor} to Figure\ref{fig:UrbanBIS}, we can rapidly grasp the main content in each scene. Furthermore, line drawings can also serve as the foundation for further artistic creation.

\section{Discussion on Limitations}

The main idea is to learn the point distribution characteristic of a specific dataset to achieve distinguished performance compared to models trained on datasets compiled using different techniques. We have validated our method on both CAD model datasets and real-scanned datasets, and the superior results demonstrate its effectiveness and advantage. 

However, to further validate the performance of our OSFENet, we also tested it on another object dataset, \textit{i.e.} SHREC, which consists of models acquired by different scanners and techniques. The training model and the predictions of our OSFENet, EC-Net\cite{Yu2018ECNet}, and NerVE\cite{Nerve2023CVPR} are presented in Figure \ref{fig:limitation}. As shown in Figure \ref{fig:limitation}, although some non-features in the vicinity of edges are erroneously taken as edge points, our method can still accurately extract the sharp features of the models. However, both EC-Net \cite{Yu2018ECNet} and NerVE \cite{Nerve2023CVPR} fail to extract sufficient sharp features describing the silhouettes of the models. 


==> 11._biography.tex <==
\vspace{-25mm}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Headshot/tuzhikun.jpg}}]{Zhikun Tu}
received the B.S. degree from Northwest University
of China in 2022. He is currently working toward the M.S
degree in software engineering with the School of Information Science and Technology, Northwest University of China. His research
interests include point cloud processing and Deep learning. 
\end{IEEEbiography}
\vspace{-25mm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Headshot/zhangyuhe.jpg}}]{Yuhe Zhang}
(Member IEEE) received the B.S. degree in software engineering and Ph.D. degree in computer applied technology from Northwest University of China in 2012 and 2017. From July 2017 to July 2020, she was a lecturer at School of Information Science and Technology, Northwest University of China. Since August 2020, she has been an Associate Professor at the School of Information Science and Technology, Northwest University of China. Her research interests include computer graphics, point cloud processing, and the digital restoration of cultural heritage.
\end{IEEEbiography}
\vspace{-25mm}

% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Headshot/Li Zhi.jpg}}]{Zhi Li} received the B.S. degree from Northwest University of China in 2022. He is currently working toward the M.S. degree in software engineering with the School of Information Science and Technology, Northwest University of China. His research interests include 3D scene generation, deep learning and point cloud processing.
% \end{IEEEbiography}
% \vspace{-25mm}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Headshot/jiayiou.jpg}}]{Yiou Jia}
received his B.S. degree in software engineering from Northwest University of China in 2022. He is currently working toward the M.S
degree in software engineering with the School of Information Science and Technology, Northwest University of China. His research interests include point cloud processing and point-based 3D object detection.
\end{IEEEbiography}
\vspace{-25mm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Headshot/likang.png}}]{Kang Li}
received the PhD degree in computer software from Northwest University, Xi’an, China, in
2013. He is currently a professor with the
School of Information Science and Technology, Northwest University. His current research interests include
intelligent information processing and visualization.
\end{IEEEbiography}
\vspace{-25mm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Headshot/daniel.png}}]{Daniel Cohen-Or}
received the BSc degree in both mathematics and computer science, in
1985, the MSc degree in computer science from Ben-Gurion University, in 1986, and the PhD degree from the Department of Computer Science,
State University of New York at Stony Brook, in 1991. He is a professor with the Department of Computer Science, Tel Aviv University. His research interests include computer graphics,
visual computing and geometric modeling and including rendering and modeling techniques, shape analysis, shape creation and editing, 3D reconstruction, photo processing, compression and streaming techniques, visibility, point set representation, morphing, and volume graphics.
\end{IEEEbiography}
\vspace{-25mm}


==> 9._add_res.tex <==
\section{Additional results on real-scanned datasets}

\begin{figure*}
  \centering
  \includegraphics[width=\linewidth]{Figure/ComparisonSupp.pdf}
  \caption{Results on the real-scanned datasets, which are produced by OSFENet, EC-Net\cite{Yu2018ECNet} and NerVE\cite{Nerve2023CVPR}.}
  \label{fig:comparison}
\end{figure*}

\subsection{Comparison with competitors}

We choose EC-Net\cite{Yu2018ECNet} and NerVE\cite{Nerve2023CVPR} as baselines for comparison on real-scanned datasets, as they achieved the first and second highest scores on the ABC dataset. Figure \ref{fig:comparison} presents the testing results of our OSFENet, EC-Net\cite{Yu2018ECNet} and NerVE\cite{Nerve2023CVPR}, on the real-scanned datasets. 

It can be observed that the EC-Net only extracts extremely sharp features, while it misses all the smooth ones. This is because EC-Net primarily focuses on sharp edges. Unlike the ABC dataset, indoor and outdoor scenes display a wider range of scales and diverse levels of detailed features, presenting additional challenges. Regarding the most recent method, NerVE, nearly all feature points are disregarded due to the normalization and voxelization operations. Achieving effective results becomes difficult when attempting to set a consistent voxel scale for models of various sizes, particularly for outdoor scenes. However, our OSFENet still performs better on these real-scanned datasets.



\subsection{Additional results}
For a specific dataset, by learning the labeled segments of the scene, the proposed OSFENet can achieve satisfactory results for predicting the features of the models from that dataset. Here, we present additional results on the aforementioned real-scanned datasets, including the indoor scene dataset S3DIS \cite{Armeni20163DSP}, as well as the outdoor scene datasets like Semantic3D \cite{Hackel2017Semantic3DnetAN} and UrbanBIS \cite{Yang2023UrbanBISAL}.

Indoor scenes and outdoor scenes differ in scale, shape, sampling density, and noise distribution. Furthermore, these two outdoor scenes exhibit features with varying scales, shapes, and levels of detail. Specifically, the buildings in Semantic3D exhibit both sharp and smooth features, whereas the buildings in UrbanBIS showcase more massive and detailed features. Furthermore, the size of building instances varies in outdoor scenes. For example, in UrbanBIS, it ranges from less than 2m to more than 100m. 

As can be seen from Figure \ref{fig:indoor} to Figure \ref{fig:UrbanBIS}, the proposed OSFENet produces superior results on these real-scanned datasets with different characteristics.


\begin{figure*}
  \centering
  \includegraphics[width=\linewidth]{Figure/indoor-spp1.pdf}
  \caption{Results of feature detection on the S3DIS dataset\cite{Armeni20163DSP}. The red points and gray points are training features and non-features, and the black points are the predicted features obtained by the proposed OSFENet.}
  \label{fig:indoor}
\end{figure*}

\begin{figure*}
  \centering
  \includegraphics[width=\linewidth]{Figure/Semantic3D-supp1.pdf}
  \caption{Results of feature detection on the Semantic3D dataset\cite{Hackel2017Semantic3DnetAN}. The red points and gray points are training features and non-features, and the black points are the predicted features obtained by the proposed OSFENet.}
  \label{fig:Semantic3D}
\end{figure*}


\begin{figure*}
  \centering
  \includegraphics[width=\linewidth]{Figure/UrbanBIS-spp1.pdf}
  \caption{Results of feature detection on the UrbanBIS dataset\cite{Yang2023UrbanBISAL}. The red points and gray points are training features and non-features, and the black points are the predicted features obtained by the proposed OSFENet.}
  \label{fig:UrbanBIS}
\end{figure*}

